Tokenized Model: A Blockchain-Empowered Decentralized Model Ownership Verification Platform

With the development of practical deep learning models like generative AI, their excellent performance has brought huge economic value. For instance, ChatGPT has attracted more than 100 million users in three months. Since the model training requires a lot of data and computing power, a well-performing deep learning model is behind a huge effort and cost. Facing various model attacks, unauthorized use and abuse from the network that threaten the interests of model owners, in addition to considering legal and other administrative measures, it is equally important to protect the model's copyright from the technical means. By using the model watermarking technology, we point out the possibility of building a unified platform for model ownership verification. Given the application history of blockchain in copyright verification and the drawbacks of a centralized third-party, this paper considers combining model watermarking technology and blockchain to build a unified model copyright protection platform. By a new solution we called Tokenized Model, it protects the model's copyright by reliable ownership record and verification mechanism. It also promotes the financial value of model by constructing the model's transaction process and contribution shares of a model. In the typical case study, we also study the various performance under usual scenario to verify the effectiveness of this platform.

==> related_work.tex <==
% This file is the text of chapter 2--Related Work

==> related_works_re.tex <==
Watermarking is often embedded into digital resources to protect copyright or from data leakage. The watermark can tell us the information of leakers and or the other concerned with the copyright.  However, due to black box nature of deep learning models, traditional methods cannot insert watermarks into models without affecting their original functions. Therefore, model watermarking technology has attracted many researchers. The current model watermarking method integrates the watermark embedding process into the training process and avoids affecting the original function of the model through the training process by designing the specific loss function. Below, we introduce three main type of model watermarking:
(1) Backdoor watermarks: Originates from backdoor attacks,
where the attacker merges a designed trigger into
the training dataset and identifies the samples containing the
trigger as a specific label instead of their true labels during the model training process. Therefore, the model will generate malicious result for the trigger-contained data and tend to be normal facing normal data. In the model watermarking method, this trigger can be seen as a non-visible watermark and by observing the model’s output for the samples containing the trigger, we can know whether the model contains the watermark or not. (2) Parameter features:
Inspired by traditional methods, where we hide the watermark into the parameters of the model. We can decode and get the watermark by a specific designed decoding process. As mentioned earlier, since it is not clear how changing model-specific parameters will affect the neural network function,
some optimization or deep learning methods are still needed
to assist the embedding process to ensure that the functionality
of the model is not affected. The advantage of this approach
is that the watermark is more stable and can hide information into models. (3) Generated object: Designed for generative models. The generative modules
like VAE and GAN of  generative models can be trained so that the
generators contain special watermarks that can be detected by
decoders.  We can verify the origin of a generative content by detecting the existence of the watermark. 

